NeuroFlow: Development of lightweight and efficient model integration scheduling strategy for autonomous driving system

This paper proposes a specialized autonomous driving system that takes into account the unique constraints and characteristics of automotive systems, aiming for innovative advancements in autonomous driving technology. The proposed system systematically analyzes the intricate data flow in autonomous driving and provides functionality to dynamically adjust various factors that influence deep learning models. Additionally, for algorithms that do not rely on deep learning models, the system analyzes the flow to determine resource allocation priorities. In essence, the system optimizes data flow and schedules efficiently to ensure real-time performance and safety. The proposed system was implemented in actual autonomous vehicles and experimentally validated across various driving scenarios. The experimental results provide evidence of the system's stable inference and effective control of autonomous vehicles, marking a significant turning point in the development of autonomous driving systems.

==> Pseudocode.tex <==
\begin{algorithm}
    \label{algorithm: pseudocode}
    \caption{Pseudocode of the NeuroFlow Scheduling System}
    \begin{algorithmic}[1]
        \State Initialize DNN queue, Non-DNN queue
        \State Process programs of DNN queue and programs in Non-DNN queue in parallel
        \For{each program $p$}
            \State $computer\_status \gets$ get\_computer\_status()
            \If{program\_uses\_DNN($p$)}
                \State Add $p$ to DNN queue
                \State $predicted\_platform \gets$ \\ \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}predict\_runtime($p$, $computer\_status$)
                \State Execute $p$ on $predicted\_platform$
            \Else
                \State Add $p$ to Non-DNN queue
                \If{is\_DAG($p$)}
                    \State Set higher priority for $p$
                \EndIf
                \State Schedule $p$ using CFS
            \EndIf
        \EndFor
    \end{algorithmic} 
\end{algorithm}

==> relatedworks.tex <==
\section{Related Works}

Autonomous vehicles are equipped with an array of sensors (e.g., cameras, LiDAR, radar, GPS) and are powered by ECUs or computational units. The advent of multi-modal networks in recent years has seen a convergence of sensors of varying modalities into a single unit. In such cases, there is a demand for data traffic up to ~2 GB/s, necessitating various hardware components \cite{SelfDrivingModule}. To facilitate this, several chip-based accelerators have been introduced, notably GPUs, NPUs, or deep learning accelerators provided by specific companies \cite{Lin2018TheAI}.

According to our research, the paper by \cite{10.1145/3492321.3519576} was the first to apply an AI system architecture to autonomous driving systems.

While there have been several proposals for communication and core modules (perception, prediction, path planning, and control) platforms based on Service Level Objectives \cite{Casini2019ResponseTimeAO, quigley2009ros}, there has been a growing interest in comprehensive system frameworks capable of handling diverse pipelines, given the emergence of large-scale models and services that need to process a substantial number of queries. Thus, we aim to build upon the research conducted by Gog et al.

\subsection{Post-training Quantization}

Post-training quantization is the technique of reducing the precision of a pre-trained deep neural network, often for the dual benefits of reduced memory footprint and computational efficiency without the need for retraining the entire network. Recent developments have steered toward more advanced quantization techniques, aiming to minimize the loss of accuracy. \cite{banner2019post}

\subsection{Middleware in Autonomous Systems}
Middleware provides a bridge between the application layer and the underlying hardware in computing systems. In the context of self-driving systems, middleware plays a pivotal role in ensuring that different components, from perception to control, can seamlessly communicate and coordinate. An optimized middleware can reduce data transfer overheads, thereby speeding up the processing time and ensuring that the self-driving system operates in real-time. Notably, there are platforms like Apollo's CyberRT\cite{apolloplatform} and the ROS Foundation's ROS1 and ROS2\cite{quigley2009ros, Casini2019ResponseTimeAO}. These systems encompass Inter-process communication and libraries for handling diverse sensor data structures. Additionally, they provide support for data and scheduling of individual modules when needed.

\subsection{Deep Learning Serving Systems}

Deep Learning Serving Systems are platforms designed to facilitate the deployment of trained deep learning models into production settings. In the context of autonomous driving, where decision-making needs to occur within milliseconds, an effective serving system is paramount. \cite{ma2020rammer} introduced a compiler for deep learning models, demonstrating performance improvements of up to threefold in inference through Data Flow Graph optimization. This underscores the ongoing efforts in system-level optimization during the inference stage and strategies for efficient model serving.

\subsection{Runtime Prediction}
When inferring from multiple deep learning models, loading them onto accelerators, or performing generic pre-processing tasks necessary for inference, it is essential to have a metric representing the expected or predictive performance of the model for each platform. Consequently, there's an emerging field focusing on predicting runtime based on the model's configuration and input. The conventional approach is to estimate the prediction runtime of deep learning models to inform inference scheduling \cite{yeung2021horus}. There have also been studies that implement real-time query processing through cluster load balancing based on the query, model, and GPU performance metrics \cite{xiao2018gandiva}.
Such runtime prediction emphasizes performance enhancement and process improvement through the optimal selection of deep learning workloads and accelerators by the scheduler. Recent scheduler or compiler methods anticipate utilizing runtime prediction as initial values for prior knowledge about the execution environment and the model.
